Classifying sequences by combining context-free grammars and OWL ontologies

This paper describes a pattern to formalise context-free grammars in OWL and its use for sequence classification. The proposed approach is compared to existing methods in terms of computational complexity as well as pragmatic applicability, with examples in the music domain.

==> fixes.tex <==
R1:
Fig 3: there is a typo Fig.2 is referenced instead of Fig.3 (pg7 last sentence) 
    -> OK
Q1: simpler cases of CFG-DL may avoid inverse properties. This would make the ontology within SROEL DL (OWL-EL) which is polinomial. 
    -> specified in section 5.1
Rolification: agreed 
    -> specified at start of Section 5

Q2/Q3: DL-reasoning is NEXP. The number of axioms (n1) formalising a CFG grows exponentially with its productions. Sequence classification axioms (n2) are constant, instead. By delegating parsing to an external tool, n is always n2. The experiment shows that combining existing parser with DL reasoning only for sequence classification has polynomial complexity (with best case down to linear). Experiments using the hybrid approach are 3 order of magnitude faster - to be reported in the paper. We can enlarge fonts of Fig5.
    -> updated figure (fonts are still hard to read but better caption). 

R2:
Constructive proof 4 -> proof of Theorem 1
    -> OK - better specified Section 4 start

Q3: Q3: by checking whether it produces the expected outputs. We use the set of classes and sequences identified by [23] as test set (cf. Table 1) - to be clarified in the paper (Sec 6). 
    -> Added in Section 6.1 (before "In order to better highlight ...")

R3:
Q1: In the paper we mention bio-informatics (e.g. genome classification). Another use case is software code classification (as programming language have CFGs), including classifying design patterns. We can briefly address them in the paper. 
    -> Section 7 (very very very very brief)


==> sections/6_results.tex <==
\section{Results}
\label{sec:results}


TBD
